Where is Physical RSI capability from? An Observational Scaling Law of LLM-as-policy

In this paper, we systematically investigate the mechanisms, scaling behavior, and generalization of physical Recursive self-improvement. We introduce PhysRSI-eval to quantify physical RSI through a five-axis metric: First-Attempt Performance, Efficiency, Success, Budget and Improvement from failure. Different VLMs are evaluated on 18 manipulation tasks under a fixed interaction budget. The analysis of experimental results motivates the Physical Barrel Hypothesis: different capabilities may constrain different parts of improvement. The five-axis metrics also distinguish systems with close public benchmark averages and show that high scores need not come with early or efficient gains. We study observational scaling from two perspectives: predicting the relative performance of VLM agents from their public capabilities, and forecasting later progress from early physical feedback. Together, these analyses ask how quickly and how far an agent can improve. Moreover, we conduct workspace interventions and then analyze what improvement leaves behind. Removing history reduces late-round success, frozen workspaces remain useful on unseen layouts, and three cross-task cases achieve success earlier. The results suggest that scene-specific adaptation and reusable experience can coexist.

==> figures_src/a1-barrel.tex <==
% Preserve the association matrix and barrel artwork; replace only A1 labels.
\begin{tikzpicture}[x=1bp,y=-1bp,text={rgb,255:red,0;green,17;blue,80}]
  \node[anchor=north west,inner sep=0] at (0,0)
    {\includegraphics[width=1610bp]{\VTwoRoot assets/barrel_matrix.png}};
  \fill[white] (550,134) rectangle (657,179);
  \node[anchor=west,inner sep=0,align=left,font=\fontfamily{phv}\selectfont\fontsize{17bp}{19bp}\selectfont]
    at (552,156) {First-Attempt\\Performance};
  \definecolor{aonebarrelbg}{RGB}{235,242,246}
  \fill[aonebarrelbg] (1348,134) rectangle (1568,173);
  \node[anchor=west,inner sep=0,align=left,font=\fontfamily{phv}\selectfont\fontsize{18bp}{19bp}\selectfont]
    at (1353,153) {First-Attempt\\Performance};
  \fill[white] (52,582) rectangle (329,613);
  \node[anchor=west,inner sep=0,font=\fontfamily{phv}\selectfont\bfseries\fontsize{20bp}{22bp}\selectfont]
    at (59,598) {A1 First-Attempt Performance};
\end{tikzpicture}%


==> figures_src/a1-radars.tex <==
% Preserve all seven radar profiles and replace their top-axis labels.
\begin{tikzpicture}[x=1bp,y=-1bp]
  \node[anchor=north west,inner sep=0] at (0,0)
    {\includegraphics[width=1280bp]{\VTwoRoot assets/radar_7models.PNG}};
  \foreach \x/\y in {160/85,480/85,800/85,1120/85,320/476,640/476,960/476} {
    \fill[white] (\x-135,\y-13) rectangle (\x+135,\y+13);
    \node[inner sep=0,text={rgb,255:red,52;green,64;blue,84},
      font=\fontfamily{phv}\selectfont\fontsize{20bp}{22bp}\selectfont]
      at (\x,\y) {First-Attempt Performance};
  }
\end{tikzpicture}%


==> figures_src/a1-teaser.tex <==
% Replace only the A1 labels; coordinates follow the original image pixels.
\begin{tikzpicture}[x=1bp,y=-1bp]
  \node[anchor=north west,inner sep=0] at (0,0)
    {\includegraphics[width=1461bp]{\VTwoRoot assets/teaserv2.jpg}};
  \definecolor{aoneteaserbg}{RGB}{240,250,252}
  \definecolor{aoneteaserradarbg}{RGB}{235,251,243}
  \fill[aoneteaserbg] (88,54) rectangle (317,81);
  \node[anchor=west,inner sep=0,font=\fontfamily{phv}\selectfont\fontsize{19bp}{21bp}\selectfont]
    at (92,68) {First-Attempt Performance};
  \fill[aoneteaserradarbg] (1092,418) rectangle (1443,447);
  \node[inner sep=0,font=\fontfamily{phv}\selectfont\fontsize{20bp}{22bp}\selectfont]
    at (1270,434) {A1. First-Attempt Performance};
\end{tikzpicture}%


==> sec/0_abstract.tex <==
\abstract{
We introduce \methodname, a benchmark that evaluates Code-as-Policy agents under a fixed trial budget of one zero-shot round (K0) and at most 17 self-improvement rounds (K1--K17) on 18 RoboDojo manipulation tasks. Existing embodied Code-as-Policy evaluations report endpoint success over independent attempts or wall-clock budgets and do not separate the zero-shot prior from gains acquired by improving on judged failures. \methodname gives every system the same tool interface and a persistent workspace of skills, tools, policy and memory, stops each task chain at its first native success, and summarizes it by a six-axis capability profile (zero-shot prior, solve chain, native score, improvement shape, execution efficiency, resource cost) whose permutation-averaged radar area is independent of spoke order. We evaluate GPT-6 Astra, GPT-6.1 Sol, Claude Opus 5.5 and Claude Sonnet 5.5 over 646 rounds with task-paired bootstrap uncertainty. Zero-shot mean scores of 0.09--0.26 rise to 0.69--0.84 at the last observed round within 17 self-improvement rounds, yet the systems differ mainly in how fast and how far they improve: Astra reaches 90\% of its own gain by K5, Sol by K7, Opus and Sonnet by K14 and K13; the composite ranks Astra above Sol (bootstrap probability 0.999) and leaves the Opus/Sonnet pair undecidable (0.77).
}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
  \centering
  \IfFileExists{assets/fig1_workflow.pdf}{\includegraphics[width=\textwidth]{assets/fig1_workflow.pdf}}{}
  \caption{\textbf{Two stages, one interface.} (a)~Zero-shot round K0 (evaluate stage, Context protocol): one episode through the shared MCP tools, no workspace or program execution. (b)~Self-improvement rounds K1--K17 (optimize stage, Harness protocol): a persistent workspace, empty at K1, from which each round runs, is graded, revised (robot actions closed) and committed, until the first native success or K17. Gray: shared interface and grading; blue: one episode; orange: the workspace and everything that edits it, absent from (a). Observe that the robot interface is identical and only the workspace loop differs.}
  \label{fig:workflow}
\end{figure*}

A recent study shows GPT-6 Astra driving RoboDojo manipulation tasks with self-written control code over direct end-effector targets---and records a self-written fix that worked once and failed on the repeat~\cite{galbotteam2026astraembodied}. Code as Policies~\cite{liang2022codeaspolicies} has grown from few-shot programs over hand-built primitives into agents that command end-effector poses and debug their own programs in simulation~\cite{galbotteam2026astraembodied,lyu2026codeactionbench,diao2026liberoagent,yang2026robotworld}. This raises a question current evaluations leave open: where does the capability come from---the model's zero-shot prior, or its ability to improve by trial and error under a bounded budget?

Eventually solving a task after many attempts is not learning: with constant per-attempt success probability $p$, the chance of at least one success in $K$ attempts, $1-(1-p)^K$, rises with $K$ while nothing is learned (83\% at $K=17$ for $p=0.1$). Endpoint success under a generous budget therefore conflates search with self-improvement; separating them requires the shape of the improvement---how fast, how far, at what cost---and a control that carries nothing between attempts. Prior embodied Code-as-Policy benchmarks score independent attempts or wall-clock budgets~\cite{fu2026capx,lyu2026codeactionbench,diao2026liberoagent,zhang2026vabench,yang2026robotworld,shen2026embodiedswe,ma2026rlebench}, and the self-evolution benchmarks that measure improvement are digital and, as far as their published descriptions state, lack a physical outcome verifier~\cite{huang2026evobench,wu2026harnessdev,singh2026agentplasticity,zheng2026seagym,xue2026pastbench,lin2026harnessupdating} (\cref{sec:related_work}). To our knowledge, none fixes a small, countable budget of judged physical attempts, lets the model carry its own code and notes between them, and reports the improvement curve with its cost.

We therefore introduce \methodname (\cref{fig:workflow}), which runs 18 dual-arm RoboDojo manipulation tasks in two stages over one tool interface (MCP). The zero-shot round (K0; the \emph{evaluate} stage, Context protocol) is one episode with no workspace, program execution or cross-episode feedback. The self-improvement rounds (K1--K17; the \emph{optimize} stage, Harness protocol) add a round loop and a persistent workspace, empty at K1, that the agent revises after each native grade (robot actions closed) and commits. A chain stops at its first native success or at K17: every system faces the same budget of judged attempts. Because K1 also introduces the harness tools, the K0$\to$K1 step is a protocol-plus-improvement step and K1--K17 is the self-improvement segment; we use recursive self-improvement (RSI) narrowly: a frozen model revises its own policy artifacts from graded outcomes, no weights change, and the improver is not improved. Whether the segment reflects learning rather than resampling is examined with the no-history control in~\cref{sec:exp-ablation} and bounded in~\cref{sec:limitations}.

We summarize a system by a six-axis capability profile: zero-shot prior, first attempt and solve chain, native score and partial progress, improvement magnitude and shape, execution efficiency, and resource cost. Every axis is normalized by protocol constants (17-round budget, per-task step limit, $[0,1]$ native score), so adding a system changes no existing score. The axes combine into a radar area $\bar A$ averaged over all spoke orders; because four axes share the first-success-round signal under the stop rule, a cluster-downweighted area serves as a control.

We evaluate GPT-6 Astra, GPT-6.1 Sol, Claude Opus 5.5 and Claude Sonnet 5.5 over 646 rounds. Under this protocol, most of each system's final score accrues after the zero-shot round (\cref{fig:curves}): the task-mean score rises from 0.09--0.26 at K0 to 0.69--0.84 at the last observed round, and 11--15 of 18 tasks are solved. The systems differ mainly in how fast and how far they improve: single chains show distinct shapes---fast and far (Astra), high start and low ceiling (Sol), slow but persistent (Opus)---and reach 90\% of their own gain between K5 and K14. An Astra-only ablation that wipes the workspace every round reaches 8\% late-round success against 42\% with it, which supports reading the K1--K17 gains as improvement rather than resampling (one system, six tasks and a different protocol;~\cref{sec:exp-ablation}). The composite orders Astra $>$ Sol $>$ \{Opus $\approx$ Sonnet\}, with $P(\text{Astra}>\text{Sol})=0.999$ and the last pair undecidable. All conclusions are limited to 18 tasks with one chain each and compare model-plus-configuration systems, not frozen models.

Finally, following observational scaling~\cite{ruan2024observational}, we outline a framework---not yet a result---for a principal component analysis (PCA) of public benchmark scores against the composite, with coding, spatial reasoning, logical and causal reasoning, and long-context handling as hypothesized abilities; with four to six closed systems it is descriptive (\cref{app:pca}).

Our contributions are:
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=2pt]
  \item \textbf{Benchmark.} \methodname: 18 tasks, one zero-shot round, at most 17 self-improvement rounds, a persistent self-authored workspace.
  \item \textbf{Metrics.} Six protocol-anchored axes, an independence analysis, an order-free composite with task-paired bootstrap uncertainty.
  \item \textbf{Findings.} Gains accrue in the self-improvement rounds at speeds and extents that separate the systems more than their zero-shot priors do; an Astra-only no-history control supports improvement over resampling.
  \item \textbf{Outlook.} A framework relating the composite to public benchmark abilities (results pending).
\end{itemize}


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Code-as-Policy and its benchmarks.}
Code as Policies~\cite{liang2022codeaspolicies} showed that a code-writing language model can act as a robot policy by emitting programs over perception and control primitives; its evaluation is one program per command. A series of 2026 benchmarks evaluates general-purpose models and coding agents in this role under controlled interfaces. \mbox{CaP-X}~\cite{fu2026capx} (whose core benchmark is CaP-Bench) varies perception privilege, primitive abstraction and feedback across eight tiers and reports success over 100 trials per task; its multi-turn tiers revise code inside one never-reset episode. CodeActionBench~\cite{lyu2026codeactionbench}, LIBERO-Agent~\cite{diao2026liberoagent}, VABench~\cite{zhang2026vabench} and RobotWorld~\cite{yang2026robotworld} fix a shared robot API and an independent success check, then aggregate one to three \emph{independent} rollouts per task: CodeActionBench reports coverage and consistency over three attempts whose verdicts are never returned to the agent; LIBERO-Agent scores stability (success in all three rollouts) with an episode-local workspace; VABench conditions on RGB demonstrations and revises only within an episode; RobotWorld runs one episode per model--task pair across five embodiment domains. EmbodiedSWE~\cite{shen2026embodiedswe} and RLE-Bench~\cite{ma2026rlebench} instead give a coding agent hours of simulator access (RLE-Bench also charges simulator steps) and grade what it builds; EmbodiedSWE's best-so-far score against wall-clock is the closest analog of our growth curve, and RLE-Bench asks agents to package experience for \emph{fresh} agents on held-out tasks. Closest to our setting, a study of GPT-6 Astra as an embodied policy~\cite{galbotteam2026astraembodied} drives RoboDojo tasks through direct end-effector targets of one to five control steps and records a self-written fix that succeeded once and failed on the repeat. Across this line, success is reported per episode, as best-of-$k$ or worst-of-$k$, or against wall-clock; as far as their protocols state, none counts dependent, judged attempts in which the model keeps its own code and notes, and none reports the resulting per-attempt trajectory. \methodname instead counts exactly such attempts---dependent, judged, with a self-authored workspace carried between them---and reports the per-attempt trajectory with its cost.

\paragraph{Measuring self-improvement in digital domains.}
A parallel line asks whether a model can improve its own harness or retained experience, almost entirely on software, search, office and game tasks. Evo-Bench~\cite{huang2026evobench} constructs tasks so that harness gains can be separated from base-model strength; HarnessDev~\cite{wu2026harnessdev} scores created and evolved harnesses on held-out success and token cost; Agent Plasticity~\cite{singh2026agentplasticity} defines plasticity as the efficiency of converting experience into held-out gains and finds that endpoint capability and acquisition efficiency diverge; SEAGym~\cite{zheng2026seagym} adds frozen update-validation, replay and saved snapshots and observes that frequent updates need not improve held-out performance; and \citet{lin2026harnessupdating} separate \emph{producing} useful updates from \emph{benefiting} from them, finding the former flat and the latter non-monotone in base capability. Related designs test experience pathways, matched retained-memory controls, cross-task ability transfer, token-normalized gains, externally evolving harnesses and vague goals~\cite{shi2026s3gym,xue2026pastbench,gao2026evoagentbench,jiang2026seaeval,ke2026evoharnessbench,wu2026aspire}. AI-R\&D benchmarks~\cite{wijk2024rebench,chan2024mlebench,starace2025paperbench,rank2026posttrainbench,chi2026ai4aibench} measure prerequisites of self-improvement, such as research engineering under time or compute budgets, rather than an agent improving its own behavior. Four lessons carry over, and the benchmark adopts three: the zero-shot round is scored apart from the self-improvement rounds (doing a task is not improving one's way of doing it); magnitude and shape, first-try and chain success, and efficiency and cost are separate axes (level, gain and efficiency reported apart); and a no-history control in the Astra ablation (\cref{sec:exp-ablation}) partly addresses search versus learning. The fourth---confirming visible-feedback gains on frozen held-out re-tests---is adopted only in part: the main chain stops at first native success and never re-tests, and our frozen-workspace evaluation on held-out layouts is small, so we report trial-and-error improvement under a bounded budget, not demonstrated frozen gain.

\paragraph{Observational analysis of capability sources.}
\citet{ruan2024observational} show that a principal component analysis of public benchmark scores across many models yields a low-dimensional capability space that predicts agentic performance from non-agentic benchmarks, with programming capability as the component most associated with agent performance. We borrow the methodology, not the scale: we plan to relate public leaderboard scores of the evaluated systems (benchmark set and sources in~\cref{app:pca}) to our composite by PCA. With four to six closed models and no compute information, the result will be a descriptive reading of which benchmark directions co-vary with embodied self-improvement, not a predictive fit.


==> sec/3_method.tex <==
% Section 3: benchmark, protocol and metrics.
% Integrator notes:
%  * \cite{liang2022codeaspolicies} is the verified key from refs_verified.bib (already merged into main.bib).
%  * \cite{hake1998interactive} was appended to main.bib (Crossref record for DOI 10.1119/1.18809, checked 2026-10-13).
%  * Material moved out of this section (D2 recovery form and ladder values, identity-term symbols, D5/D8 history)
%    is in paper/integration/handoff_method.tex, to be pasted into Appendix C (app:metrics) by the appendix agent.
%  * Figure 1 (fig:workflow) lives in sec/1_intro.tex.

\section{The RoboDojo-RSI Benchmark}
\label{sec:method}

\methodname measures how well a Code-as-Policy agent~\cite{liang2022codeaspolicies} performs embodied manipulation under a small, fixed number of graded attempts per task (\cref{fig:workflow}).

\subsection{Design principles}
\label{sec:design}

\paragraph{What is measured.} No weights are updated; whatever the agent learns it must write into artifacts (skills, tools, policies, memory) that it later reads back. Capability thus has two components---solving a task within one episode, and improving one's own artifacts across a short chain of graded episodes---which the benchmark separates with two stages per task: a zero-shot round (K0) and up to 17 self-improvement rounds (K1--K17), internally the evaluate/Context and optimize/Harness protocols. A \emph{round} is one graded episode (a trial), \emph{native} means returned by RoboDojo's own grader or clock, and an \emph{extra attempt} is a non-canonical rerun outside the chain (\cref{app:protocol}). The chain is capped at K17 and stops at the first native success, so that the round of first success, the partial progress before it and the physical steps spent are compared under one budget. A chain is never re-tested after its first success, so a retained skill and a one-off success are scored alike (\cref{sec:limitations}).

\paragraph{Two stages.} In the zero-shot round the model has one episode per task: it observes, acts and may correct its course, with the same per-action observations as in later rounds, but nothing outlives the episode---no workspace, program execution or reset. The self-improvement rounds add a persistent, initially empty workspace and tools to read, write and run programs in it; after each graded round the agent revises its artifacts with physical actions closed and the next round starts from the committed revision, so any improvement that is carried from one round to the next must pass through what the agent wrote down---recursive self-improvement (RSI) in our sense; chance variation between attempts remains and is addressed in~\cref{sec:exp-curves,sec:exp-ablation}. We use RSI narrowly: a frozen model revising its own policy artifacts from graded outcomes; the improver itself is not improved.

\subsection{Tasks}
\label{sec:tasks}

The benchmark uses 18 dual-arm manipulation tasks from RoboDojo~ (\cref{tab:app-tasks},~\cref{app:benchmark}), selected to span the observed difficulty range . Each task keeps its native step limit $N_t$ (300--1300 control steps at 25\,Hz) and its default scene layout (layout~0, seed~0) in every round. The native grader returns a success flag $y_{t,k}\in\{0,1\}$ and a score $q_{t,k}\in[0,1]$ with $q_{t,k}=1$ whenever $y_{t,k}=1$: six tasks are binary ($q=y$) and twelve, the graded set $\mathcal{G}$, score the highest ordered tier reached. The success check is independent of the tiers and the metrics use $q$ and $y$ unchanged (\cref{tab:app-tasks}).

\subsection{Protocol}
\label{sec:protocol}

\paragraph{Zero-shot round (K0).} The four MCP tools of~\cref{fig:workflow} are attached to a command-line coding client. On the trigger message \texttt{evaluate task} the model runs one episode, correcting freely but unable to reset, until success, the step limit or the reasoning budget; the grader returns $(q_{t,0},y_{t,0})$. K0 is run once per task (existing zero-shot results are reused rather than re-run) and nothing from it is carried into K1 .

\paragraph{Self-improvement rounds (K1--K17).} On \texttt{optimize task} the client additionally receives a workspace restricted to \texttt{skills/}, \texttt{tools/}, \texttt{policy/} and \texttt{memory/}, plus tools to read, write and run programs in it and to inspect the chain's committed rounds (\cref{fig:workflow}). At K1 the workspace is empty; the robot tools also return the public outcomes of the three most recent rounds. Round $k$ (i)~\emph{executes} one episode from the committed workspace; (ii)~is \emph{graded} natively (score, success, failure reason and mechanism); (iii)~is \emph{revised} with physical actions closed---the agent edits its artifacts and writes a round summary, effective from the next round; (iv)~is \emph{committed}, and round $k{+}1$ starts from the commit. The chain stops at the first native success or after K17, without confirmation rounds; retry and invalid-round rules are in~\cref{app:protocol}.

\paragraph{Physical interface and budgets.} An action sets a target pose for each end-effector, within 5\,cm and 0.35\,rad of its current pose, runs for 1--5 control steps at 25\,Hz and returns the robot state and three camera images (\cref{fig:workflow}). Budgets are 4200\,s of reasoning per round and 1800\,s for revision (600\,s for the two Claude systems,~\cref{app:protocol}). Each task thus has a physical budget of $17\,N_t$ steps; a round cut short by the reasoning budget counts as a failure (per-system deviations:~\cref{sec:exp-setup},~\cref{tab:app-config}).

\subsection{Metrics}
\label{sec:metrics}

\paragraph{Notation.} Rounds are indexed by $k$ ($k=0$ zero-shot, $k=1,\dots,17$ chain) and $K\in\{1,\dots,17\}$ is a round budget. $T_t=\min\{k\ge 1: y_{t,k}=1\}$ is the first-success round of task $t$ ($\infty$ if unsolved); $\ell_t(K)=\min(K,T_t)$ the last round observed within budget $K$ or, for an unfinished chain, its last observed round; $a_t$ the steps executed in the first-success episode; $\mathcal{I}$ the frozen set of tasks solved by every compared system. $C(K)=\frac{1}{18}\sum_t \mathbf{1}[T_t\le K]$ is coverage within budget $K$, $\mathrm{AUC}^{C}=\frac{1}{17}\sum_{K=1}^{17}C(K)$ its discrete area, $\bar q_k=\frac{1}{18}\sum_t q_{t,k}$ the mean score at round $k$, $\bar x(K)=\frac{1}{18}\sum_t q_{t,\ell_t(K)}$ the task-mean last-observed score by round $K$ (the growth curve of~\cref{sec:exp-curves}), and $R$ the fraction of tasks failed at K1 but solved by K17.

\paragraph{D1: zero-shot prior.} The mean native score of the zero-shot round,
\begin{equation}\label{eq:d1}
D_1=\bar q_0=\frac{1}{18}\sum_{t=1}^{18} q_{t,0}=C(0)+\bigl(1-C(0)\bigr)\,F(0),
\end{equation}
with $C(0)=\frac{1}{18}\sum_t y_{t,0}$ the K0 success rate and $F(0)$ the mean partial score over K0 failures; D1 is the only axis computed from K0.

\paragraph{D2: first try and solve chain.} Each task earns a utility from its first-success round,
\begin{align}
u_t&=\tfrac{1}{3}\Bigl(\mathbf{1}[T_t{=}1]+\mathbf{1}[T_t{\le}17]+\mathbf{1}[T_t{\le}17]\,\tfrac{18-T_t}{17}\Bigr),\nonumber\\
D_2&=\frac{1}{18}\sum_{t=1}^{18}u_t=\frac{C(1)+C(17)+\mathrm{AUC}^{C}}{3},\label{eq:d2}
\end{align}
and~\cref{app:metrics} separates first-try success from recovery after a K1 failure.

\paragraph{D3: native score and partial progress.} On the graded set, the area under the best-so-far score curve $b_t(K)=\max_{1\le k\le \ell_t(K)} q_{t,k}$,
\begin{equation}\label{eq:d3}
D_3=\frac{1}{|\mathcal{G}|}\sum_{t\in\mathcal{G}}\frac{1}{17}\sum_{K=1}^{17} b_t(K),
\end{equation}
the binary coverage area on graded tasks plus the partial-score area accrued before success or while unsolved (\cref{app:metrics}).

\paragraph{D4: improvement magnitude and growth shape.} The headroom-normalized gain over K0 (Hake's normalized gain~\cite{hake1998interactive}), averaged over budgets,
\begin{align}
x_t(K)&=q_{t,\ell_t(K)},\qquad
NG(K)=\frac{\sum_t\bigl[x_t(K)-q_{t,0}\bigr]}{\sum_t\bigl(1-q_{t,0}\bigr)},\nonumber\\
D_4&=\operatorname{clip}_{[0,1]}\!\Bigl(\frac{1}{17}\sum_{K=1}^{17} NG(K)\Bigr)=NG(17)\times\Phi,\label{eq:d4}
\end{align}
where $NG(17)$ is the fraction of the K0 gap closed by K17 and $\Phi=D_4/NG(17)\in[\tfrac{1}{17},1]$ a shape factor (how early the gain is realized and whether it is held).

\paragraph{D6: execution efficiency.} On the common-success set, one minus the geometric mean of the step fraction used by the first-success episode,
\begin{equation}\label{eq:d6}
D_6=1-\exp\!\Bigl(\frac{1}{|\mathcal{I}|}\sum_{t\in\mathcal{I}}\ln\frac{a_t}{N_t}\Bigr),
\end{equation}
so that ratios of $1-D_6$ equal paired geometric-mean step ratios.

\paragraph{D7: resource cost.} Physical resources spent from K1 to the end of the solve window ($T_t$ if solved, else the last observed round), in full-budget attempts,
\begin{align}
U_t&=\tfrac{W_t+Z_t}{N_t}+e_t,\quad
s_t=\mathbf{1}[T_t{\le}17]\max\bigl(0,1-\tfrac{U_t}{17}\bigr),\nonumber\\
D_7&=\frac{1}{18}\sum_{t=1}^{18} s_t=\mathrm{AUC}^{C}-\delta,\label{eq:d7}
\end{align}
where $W_t$ counts steps executed in canonical episodes, $Z_t$ steps not executed in failed episodes cut short by the reasoning budget (charged at the full limit) and $e_t$ recorded extra attempts, each charged one limit. D7 is the area under the cost--coverage curve over the $17\,N_t$ budget; $\delta\ge 0$ collects success-episode steps, extra attempts and truncation charge-back (\cref{app:metrics}).

\paragraph{Selection principles.} (i)~Each axis reads capability from the protocol itself and improving any single task result never lowers it (verified by perturbation); (ii)~anchors are protocol or physical constants, so every axis lies in $[0,1]$ without min--max scaling and existing scores do not change when a system is added. The labels skip D5 (the numbering gap is explained in~\cref{app:metrics}).

\paragraph{Shared information.} D1 and D6 are statistically separate from the rest (within-system bootstrap covariation at most 0.38), but under first-success stopping a solve at $T_t$ simultaneously raises coverage, realizes the gain and stops the cost, so D2, D3, D4 and D7 are four readings of the same first-success-round signal (covariation 0.69--0.93), each adding only its own term (first-try and recovery ladder, partial-score area, K0 headroom and shape factor, cost correction $\delta$).

\paragraph{Composite.} With axis scores $r_1,\dots,r_n$ ($n=6$) a system is summarized by the permutation-averaged radar area
\begin{equation}\label{eq:area}
\bar A=\frac{\bigl(\sum_i r_i\bigr)^2-\sum_i r_i^2}{n(n-1)}=\bar r^{\,2}-\frac{\sigma_r^2}{n-1},
\end{equation}
with $\bar r$ the mean and $\sigma_r^2$ the population variance of the six axis scores: $\bar A\in[0,1]$ is the mean over all axis orderings of the drawn polygon's area as a fraction of the full hexagon, hence independent of the drawing order. For the systems compared here the variance term is small, so $\bar A$ is close to the squared mean axis score and orders the four systems as the mean does (\cref{sec:exp-axes}). Because of the shared first-success signal we also report a cluster-weighted variant, with weights $1/4$ for D2, D3, D4, D7 (together one axis) and $1$ for D1, D6 in the weighted analogue of~\cref{eq:area} ; the identities behind each axis are collected in~\cref{app:metrics}. $\bar A$ is descriptive: it is not comparable across axis sets or weightings, and area ratios are not capability multiples.


==> sec/4_experiments.tex <==
\section{Experiments and Analysis}
\label{sec:experiments}

% ---------------------------------------------------------------------------
% Number sources for this section (nothing recomputed here):
%   understand/02_metrics_results_pack.md  -> axis scores + CIs, areas, pairwise bootstrap
%                                             probabilities, robustness, growth-shape numbers,
%                                             K0/K17 headline numbers, cost numbers
%   understand/04_experiments_pack.md      -> headline table, protocol heterogeneity, ablation
%                                             design/caveats, frozen held-out test
%   figures_src/fig_ablation_source_rates.csv, fig_ablation_source_contrasts.csv
%                                          -> ablation rates and contrasts (repo-derived; the
%                                             contrasts are drawn in assets/fig_ablation_contrasts.pdf)
% Wording rules: "performance-improvement curve" only (never "scaling law"); no ranking between
% Opus and Sonnet; K0->K1 is a mixed protocol-plus-improvement step; "interval excludes zero" /
% "separated" instead of "significant"; K0, K1--K17 in text mode; American spelling.
% Material trimmed from this section for the appendix is in paper/integration/handoff_experiments.tex.
% ---------------------------------------------------------------------------

We ask whether the budget improves every system (\cref{sec:exp-curves}), how the systems differ on the six axes (\cref{sec:exp-axes}) and in growth shape (\cref{sec:exp-growth}), and which parts of the loop carry the gain (\cref{sec:exp-ablation}); \cref{sec:exp-pca} outlines the pending capability-source analysis.

\subsection{Setup}
\label{sec:exp-setup}

\paragraph{Systems and runs.} We evaluate four model--configuration systems, GPT-6 Astra (xhigh), GPT-6.1 Sol (xhigh), Claude Opus 5.5 (high) and Claude Sonnet 5.5 (xhigh), written Astra, Sol, Opus and Sonnet below; four-number lists follow this order. All four see the same MCP tools, tasks and scene layout, but client (Codex CLI versus Claude Code), prompts, reasoning effort, revision window (1800\,s for Astra and Sol, 600\,s for Opus and Sonnet), image format (PNG for Astra only) and timing conventions differ, and Astra alone received three task-specific hints (scoring-structure and revision-hygiene notes on \texttt{pack\_objects\_into\_box} from K7, \texttt{store\_tools\_in\_toolbox} from K8 and \texttt{swap\_blocks} from K12; \cref{tab:app-config}); we compare systems as run, not frozen models. Each system runs one chain per task on the 18 tasks: a zero-shot round (K0, reused from the existing zero-shot runs; per-system confirmation in~\cref{app:protocol}) and up to 17 self-improvement rounds (K1--K17) that stop at the first native success, 646 canonical episodes in all (\cref{tab:app-config}). Three Sonnet chains are unfinished (last observed at K15, K15 and K11); Sonnet's estimates are observed snapshots with upper bounds assuming next-round success.

\paragraph{Uncertainty.} Unless stated otherwise, every interval and probability comes from a task-paired bootstrap over the 18 tasks ($B{=}5000$, seed 20261012; 95\% percentile intervals); $P(\text{X}>\text{Y})$ is the bootstrap probability that X's value exceeds Y's, and a difference is \emph{separated} when its interval excludes zero. The paper reports 36 axis-pair differences, six area-pair differences (each under two weightings), seven ablation contrasts (each in two windows) and two frozen-test contrasts, 51 comparisons in all, with no multiplicity correction. With one chain per task, the intervals reflect task sampling only, not run-to-run variance on a fixed task.

\paragraph{Comparability caveat.} A round cut off by the per-round inference time limit counts as a failure, and truncation was unequal: Opus lost 11/18 K0 and 9/18 K1 rounds to the limit (Sonnet 6/18 at K0; truncated failed self-improvement rounds 5 / 0 / 14 / 2), which depresses its zero-shot and early-round readings; on the task subsets untruncated for all four systems, Sol and Opus are tied.

\subsection{All four systems improve under the trial budget}
\label{sec:exp-curves}

\begin{figure}[tb]
  \centering
  \IfFileExists{assets/fig_curves.pdf}{\includegraphics[width=\columnwidth]{assets/fig_curves.pdf}}{}
  \caption{\textbf{All four systems improve within 17 self-improvement rounds, at different speeds.} (a) Performance-improvement curve: the task-equal-weight last-observed mean score $\bar x(K)$ from K0 to K17 (18 tasks, one chain each; unsolved tasks contribute their latest, not best, score, so the curve can dip). Stars mark $\tau_{90}$ (\cref{sec:exp-growth}; K5 / K7 / K14 / K13). (b) Task coverage $C(K)$ (\cref{sec:metrics}). Observe in (b) that Astra's coverage is flat after K9 and Sol's after K8, whereas Opus keeps adding tasks through K15 and overtakes Sol; Sonnet's values from K12 onward are observed snapshots (three chains unfinished).}
  \label{fig:curves}
\end{figure}

\paragraph{Claim.} Under the 17-round budget each system raises coverage and mean native score far above its zero-shot level; most of the rise happens inside the self-improvement rounds rather than at the K0$\to$K1 switch, and its size and shape separate the systems more than their zero-shot level does.

\paragraph{Result.} \Cref{fig:curves} shows the performance-improvement curves. At K0 the systems solve 3 / 3 / 1 / 1 of 18 tasks with mean scores 0.242 / 0.264 / 0.086 / 0.111; the first self-improvement round lifts this to 6 / 4 / 2 / 2 tasks, coverage reaches 15 / 12 / 13 / 11 of 18 by K17 (Sonnet's upper bound 14 / 18; \cref{tab:app-coverage}), and the last-observed mean ends at 0.842 / 0.689 / 0.744 / 0.700. The gain is not confined to the first tooled attempt: of the tasks failed at K1, 9/12, 8/14, 11/16 and 9/16 are solved later in the chain, and the K0$\to$K1 step accounts for only 30\% / 9\% / 15\% / 13\% of each system's headroom-normalized gain (axis D4,~\cref{eq:d4}).

\paragraph{Caveats.} K0$\to$K1 changes the protocol as well as the round index (K1 adds the persistent workspace and executable tools), so we treat it as a mixed protocol-plus-improvement step and attribute only K1--K17 to iterative self-improvement. Chains stop at their first success and carry the last observation forward, so $\bar x(K)$ is an observation curve, not a re-evaluation of a frozen policy. Repeated independent attempts alone raise the chance of at least one success ($1-(1-p)^{K}$ for a constant per-round probability $p$), so rising coverage is not by itself proof of learning; the only no-history control is arm A5 of the ablation (\cref{sec:exp-ablation}; Astra only, different protocol: 3/36 versus 15/36 late-round successes).

\subsection{Six-axis capability profile}
\label{sec:exp-axes}

% Source: 02_metrics_results_pack.md Sec. 3 (axis scores, CIs, separated pairs, Sonnet upper bounds).
\begin{table*}[tb]
  \caption{\textbf{Six-axis profile: Astra leads on the four chain axes; Opus and Sonnet are not separable.} Axis scores in $[0,1]$ (higher is better) with 95\% task-paired bootstrap intervals (\cref{sec:exp-setup}) below each value; best per axis in bold; the last column lists the separated pairs (interval excludes zero; ``all'' = the other three systems). Sonnet's D2, D3 and D4 are observed snapshots (upper bounds 0.4619, 0.5699, 0.5088 if its unfinished chains succeed next round). D6 uses the nine tasks solved by all four systems.}
  \label{tab:axes}
  \tablestyle{3.5pt}{1.0}
  \begin{tabular}{l r r r r l}
    \toprule
    Axis & Astra & Sol & Opus & Sonnet & Separated pairs \\
    \midrule
    D1 zero-shot prior & 0.2417 & {\bfseries 0.2639} & 0.0861 & 0.1111 & Astra $>$ Opus; Sol $>$ Opus \\
      & {\scriptsize [0.092, 0.420]} & {\scriptsize [0.108, 0.444]} & {\scriptsize [0.000, 0.214]} & {\scriptsize [0.028, 0.236]} & \\
    \addlinespace[1.5pt]
    D2 first attempt \& solve chain & {\bfseries 0.6394} & 0.4869 & 0.4346 & 0.3954 & Astra $>$ all \\
      & {\scriptsize [0.480, 0.784]} & {\scriptsize [0.307, 0.660]} & {\scriptsize [0.290, 0.580]} & {\scriptsize [0.236, 0.553]} & \\
    \addlinespace[1.5pt]
    D3 native score \& partial progress & {\bfseries 0.7951} & 0.6569 & 0.5755 & 0.5272 & Astra $>$ all; Sol $>$ Sonnet \\
      & {\scriptsize [0.611, 0.950]} & {\scriptsize [0.464, 0.835]} & {\scriptsize [0.386, 0.767]} & {\scriptsize [0.330, 0.729]} & \\
    \addlinespace[1.5pt]
    D4 improvement magnitude \& shape & {\bfseries 0.7085} & 0.4855 & 0.4919 & 0.4757 & Astra $>$ all \\
      & {\scriptsize [0.502, 0.879]} & {\scriptsize [0.262, 0.700]} & {\scriptsize [0.325, 0.659]} & {\scriptsize [0.299, 0.648]} & \\
    \addlinespace[1.5pt]
    D6 execution efficiency & {\bfseries 0.3837} & 0.3543 & 0.2975 & 0.2415 & Sol $>$ Sonnet \\
      & {\scriptsize [0.252, 0.488]} & {\scriptsize [0.266, 0.435]} & {\scriptsize [0.198, 0.396]} & {\scriptsize [0.122, 0.358]} & \\
    \addlinespace[1.5pt]
    D7 resource cost & {\bfseries 0.7025} & 0.5387 & 0.4185 & 0.4268 & Astra $>$ all \\
      & {\scriptsize [0.533, 0.848]} & {\scriptsize [0.344, 0.720]} & {\scriptsize [0.241, 0.600]} & {\scriptsize [0.255, 0.600]} & \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{figure}[tb]
  \centering
  \IfFileExists{assets/fig_radar.pdf}{\includegraphics[width=0.8\columnwidth]{assets/fig_radar.pdf}}{}
  \caption{\textbf{Six-axis profile: Astra's polygon encloses the other three on every axis except D1 (zero-shot prior, where Sol leads).} Each spoke is an axis score on fixed $[0,1]$ anchors taken from the protocol (outer ring $=1$, higher is better); the legend gives the permutation-averaged area $\bar A$, independent of spoke order. Observe that the Opus and Sonnet polygons interleave and that the systems differ least on D1 and D6.}
  \label{fig:radar}
\end{figure}

% Source: 02_metrics_results_pack.md Sec. 4 (areas, CIs, cluster-1/4) and Sec. 5 (pairwise probabilities, full-order probability).
% Placed directly after fig:radar with [t] so that it lands near its text (R3 6.1).
\begin{table}[t]
  \caption{\textbf{Radar area: Astra $>$ Sol $>$ \{Opus $\approx$ Sonnet\}.} Top: $\bar A$ (fraction of the full hexagon) with 95\% task-paired bootstrap intervals under equal and cluster-1/4 weights (\cref{sec:metrics}); ``Sonnet, completed'' assumes its unfinished chains succeed next round. Bottom: bootstrap probability that the first system has the larger area under equal ($P_{\mathrm{eq}}$) and cluster-1/4 ($P_{\mathrm{cl}}$) weights, the 95\% interval of the equal-weight difference $\Delta_{\mathrm{eq}}$, and (last row) the probability of the complete order Astra $>$ Sol $>$ Opus $>$ Sonnet.}
  \label{tab:area}
  \tablestyle{3pt}{1.0}
  \begin{tabular}{l r r}
    \toprule
    System & $\bar A$, equal & $\bar A$, cluster-1/4 \\
    \midrule
    Astra  & {\bfseries 0.3268} & {\bfseries 0.2154} \\
           & {\scriptsize [0.200, 0.467]} & {\scriptsize [0.126, 0.321]} \\
    Sol    & 0.2124 & 0.1594 \\
           & {\scriptsize [0.107, 0.345]} & {\scriptsize [0.083, 0.254]} \\
    Opus   & 0.1425 & 0.0876 \\
           & {\scriptsize [0.071, 0.238]} & {\scriptsize [0.044, 0.152]} \\
    Sonnet & 0.1276 & 0.0787 \\
           & {\scriptsize [0.061, 0.222]} & {\scriptsize [0.037, 0.139]} \\
    Sonnet, completed & 0.1444 & 0.0861 \\
    \bottomrule
  \end{tabular}

  \vspace{3pt}
  \begin{tabular}{l r r r}
    \toprule
    Pair & $P_{\mathrm{eq}}$ & 95\% CI of $\Delta_{\mathrm{eq}}$ & $P_{\mathrm{cl}}$ \\
    \midrule
    Astra $>$ Sol    & 0.999 & [0.035, 0.205] & 0.994 \\
    Astra $>$ Opus   & 1.000 & [0.096, 0.281] & 1.000 \\
    Astra $>$ Sonnet & 1.000 & [0.113, 0.291] & 1.000 \\
    Sol $>$ Opus     & 0.964 & [$-$0.005, 0.159] & 0.994 \\
    Sol $>$ Sonnet   & 0.993 & [0.016, 0.168] & 0.996 \\
    Opus $>$ Sonnet  & 0.771 & [$-$0.031, 0.058] & 0.690 \\
    Full order       & 0.736 & -- & 0.679 \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Claim.} Astra is separated from the other three on the composite and on every chain axis, not by its zero-shot prior; Sol is likely above Opus and Sonnet; the last pair cannot be ordered on 18 tasks.

\paragraph{Result.} \Cref{tab:axes} lists the axis scores and~\cref{fig:radar} draws them. Astra leads on all four chain axes, D2 (\cref{eq:d2}), D3 (\cref{eq:d3}), D4 (\cref{eq:d4}) and D7 (\cref{eq:d7}), every pairwise interval excluding zero. Sol has the highest zero-shot prior (D1,~\cref{eq:d1}: 0.264, not separated from Astra's 0.242) and is separated from Sonnet on D3 and D6 (\cref{eq:d6}); no other D6 pair is separated, so we do not rank on it. \Cref{tab:area} aggregates the axes into $\bar A$. The bootstrap ranks Astra first with probability 0.999; Sol is above Sonnet with probability 0.993 and above Opus with 0.964, but the Sol$-$Opus interval touches zero, so under equal weighting this is a likely rather than a separated lead. Opus versus Sonnet is undecidable: $P(\text{Opus}>\text{Sonnet})=0.77$, the difference interval is $[-0.031, +0.058]$, and if Sonnet's unfinished chains succeed next round its area (0.1444) exceeds Opus's (0.1425). The complete order has probability 0.736; the only ranking the data support is Astra $>$ Sol $>$ \{Opus $\approx$ Sonnet\}.

\paragraph{Robustness.} All 60 spoke orders and every leave-one-axis-out variant give the same point-estimate order (\cref{tab:app-robust}); $P(\text{Sol}>\text{Opus})$ falls to 0.875 only when D1 is dropped. D2, D3, D4 and D7 are, however, four readings of the same first-success-round information under the stop-at-first-success rule (task-level correlations 0.94--0.99), so the equal-weight area counts it four times. The cluster-1/4 weighting removes the quadruple count: areas become 0.2154 / 0.1594 / 0.0876 / 0.0787, the order is unchanged, the Sol$-$Opus lead sharpens to $P=0.994$ with an interval excluding zero, and Opus versus Sonnet stays open ($P=0.690$).

% Source: 02_metrics_results_pack.md Sec. 9 and 04_experiments_pack.md headline table (M69/M70/RESOURCE, M23); former Sec. 4.7 (Cost), merged here (R2 E3).
\paragraph{Cost.} The one like-for-like cost reading is execution efficiency on the nine tasks solved by all four systems: median first-success episode length 407 / 491 / 601 / 653 steps and a paired geometric-mean step ratio to Astra of 1.00 / 1.05 / 1.14 / 1.23; these differences are descriptive (the only D6 pair whose interval excludes zero is Sol $>$ Sonnet,~\cref{tab:axes}). Step totals, wall-clock and tokens are metered differently per vendor---full usage receipts for Sol only, output estimates for Opus and Sonnet, partial receipts (71 of 91 episodes) for Astra---and are reported with their caveats in~\cref{tab:app-cost}.

\subsection{Growth shape: inflection and persistence}
\label{sec:exp-growth}

\paragraph{Claim.} Systems that end at similar levels reach them along different paths; the inflection round and the persistence of late recoveries distinguish them where endpoints do not.

\paragraph{Result.} From $\bar x(K)$ in~\cref{fig:curves}a we read, per system, $\tau_{90}$ (the first round reaching 90\% of its own K0$\to$peak gain), the pre-inflection slope $v_{90}=(\bar x(\tau_{90})-\bar x(0))/\tau_{90}$ in score per round, and the increment uniformity $U_{90}\in[1/\tau_{90},1]$ (1 for equal steps, $1/\tau_{90}$ for a single jump); all three index speed and shape relative to each system's own start and peak, not level. $\tau_{90}$ falls at K5 / K7 / K14 / K13, with slopes 0.114 / 0.062 / 0.042 / 0.045 per round and uniformities 0.913 / 0.885 / 0.526 / 0.448. Three archetypes emerge on single chains. \emph{Astra} inflects early and plateaus: 11/18 tasks by K3 (69\% of its gain), 95\% of the gain by K5, a pre-inflection slope 1.8--2.7 times the others', and one additional task between K6 and K17. \emph{Opus} inflects late but keeps recovering: the lowest start (0.086), 7/18 tasks by K6 (56\% of its gain) and $\tau_{90}$ at K14, yet six further tasks solved after K6 (\cref{app:additional}) against one, two and five for Astra, Sol and Sonnet, the largest number of recoveries after a K1 failure (11 of 16, rate 0.688 vs.\ Sol's 8/14 = 0.571; Astra's rate is 9/12 = 0.750) and a final coverage of 13/18 above Sol's 12/18; Opus's early rounds are also depressed by inference-time truncation (\cref{sec:exp-setup}), so its late inflection is partly a budget artifact; Sonnet resembles it in timing (K13), with the least uniform increments. \emph{Sol} starts highest (0.264) and inflects early (K7) with high uniformity (0.885) but has the lowest ceiling: it closes only $\mathrm{NG}(17)=0.577$ of its K0 headroom (\cref{eq:d4}; Astra 0.791, Opus 0.720, Sonnet 0.663) and ends below Opus in coverage and last mean.

\paragraph{Scope.} These are descriptive shape statistics on single chains. On D4, which folds magnitude and shape together, the three non-Astra systems sit at 0.486 / 0.492 / 0.476 with overlapping intervals, so their order on that axis is within noise; the archetypes describe paths, not a ranking, and the uniformity reading holds only up to the 90\% crossing.

% Sources: design and caveats from 04_experiments_pack.md Sec. (c)/(d); rates from
% figures_src/fig_ablation_source_rates.csv (repo-derived). Coded before the subsection heading so that
% the float precedes fig:ablation (R3 6.2); row order follows the narrative (A0, A0F, A4R, A4, A1, A2, A5).
\begin{table}[tb]
  \caption{\textbf{Ablation design and late-round success (Astra, six tasks $\times$ two replicate chains, rounds K1--K6, no first-success stop).} W: workspace persists; O: outcome details after each round (score, failure reason, prior outcomes; the binary success flag is visible to every group); Img / Log: prior-round images / action logs. Every group sees a new layout each round (same sequence in every group) except A0F, which keeps its first layout and is descriptive only. Success is successes / observed rounds over K4--K6 (A4R lacks one K6 round; per-round counts in~\cref{tab:app-ablation-rounds}); A4 was cancelled. Paired contrasts: \cref{fig:ablation}.}
  \label{tab:ablation}
  \tablestyle{2pt}{1.0}
  \begin{tabular}{l l c c c c r}
    \toprule
    Group & Role & W & O & Img & Log & K4--K6 \\
    \midrule
    A0  & full loop               & \cmark & \cmark & \cmark & \cmark & 15/36 (42\%) \\
    A0F & full loop, fixed layout & \cmark & \cmark & \cmark & \cmark & 22/36 (61\%) \\
    A4R & workspace + feedback    & \cmark & \cmark & \xmark & \xmark & 16/35 (46\%) \\
    A4  & workspace only          & \cmark & \xmark & \xmark & \xmark & cancelled \\
    A1  & no images               & \cmark & \cmark & \xmark & \cmark & 12/36 (33\%) \\
    A2  & no outcome details      & \cmark & \xmark & \cmark & \cmark & 5/36 (14\%) \\
    A5  & no history              & \xmark & --     & \xmark & \xmark & 3/36 (8\%) \\
    \bottomrule
  \end{tabular}
\end{table}

% Contrast source: figures_src/fig_ablation_source_contrasts.csv (repo-derived; the four K4--K6 contrasts
% vs A0 are verbatim from analysis/remote/ablation_contrasts.json, the rest recomputed with the same
% task-cluster procedure, seed 20261011, B = 20000). The master doc (article_final.md, Results) reports
% narrower intervals (e.g. A4R-A5 +18 [+4,+33], A0-A5 +24 [+4,+43]) and A4R = 20/72, 17/36; those likely
% came from a chain-level bootstrap and count the missing A4R K6 round as a success. Not used here.
% Figure: figures_src/fig_ablation_contrasts.py (contrasts panel only; the former rates panel is tab:ablation).
\begin{figure}[tb]
  \centering
  \IfFileExists{assets/fig_ablation_contrasts.pdf}{\includegraphics[width=\columnwidth]{assets/fig_ablation_contrasts.pdf}}{}
  \caption{\textbf{Ablation contrasts: only history-versus-no-history is distinguishable from zero.} Groups as in~\cref{tab:ablation}. Paired differences of task-level mean success (percentage points) over K1--K6 (light) and K4--K6 (dark), with 95\% task-cluster bootstrap intervals over six tasks ($B{=}20\,000$, no multiplicity correction); filled markers exclude zero. Observe that A4R$-$A5 and A0$-$A5 are positive in both windows, whereas removing images or outcome details, adding raw records and fixing the layout all include zero, and the A0$-$A4R contrast changes sign between windows.}
  \label{fig:ablation}
\end{figure}

\subsection{What the workspace and feedback contribute (ablation)}
\label{sec:exp-ablation}

\paragraph{Claim.} In this Astra-only ablation, carrying a workspace and outcome feedback across rounds is what separates improvement from repeated independent attempts; whether the finer history channels (score and failure reason, images, action logs) add to that cannot be resolved at this sample size.

\paragraph{Setup.} The ablation runs on Astra only (xhigh), on six of the 18 tasks (\texttt{push\_T}, \texttt{plug\_in\_charger}, \texttt{deposit\_coin}, \texttt{play\_Xylophone}, \texttt{pour\_by\_language}, \texttt{pour\_liquid\_into\_cup}) with two replicate chains per task (12 chains per group); rounds K1--K6 are all run with a mandatory revision after each round (no first-success stop) and, unlike the main benchmark, the scene layout changes every round (schedule in~\cref{app:additional}). \Cref{tab:ablation} gives the factor design; A4 (workspace only) was cancelled, so only pairwise differences are reported, paired across groups by (task, replicate); the pre-registered primary readout is success over K4--K6, with K1--K6 also reported. With six task clusters the intervals are wide and the analysis is exploratory; the minimum detectable difference of roughly 25--35\,pp means that an interval containing zero reads ``not detected'', not ``no effect''.

\paragraph{Result.} \Cref{fig:ablation} gives the outcome. Late-round success is 3/36 (8\%) with no history (A5), 15/36 (42\%) with the full loop (A0) and 16/35 (46\%) with workspace and feedback only (A4R). The two history contrasts are the only ones whose intervals exclude zero in both windows: A4R$-$A5 is $+17$\,pp [$+4$, $+31$] over K1--K6 and $+42$\,pp [$+17$, $+69$] over K4--K6; A0$-$A5 is $+24$\,pp [$+3$, $+46$] and $+33$\,pp [$+11$, $+64$]. Every other contrast---removing outcome details or images, adding raw records on top of feedback, adding logs alone, fixing the layout---includes zero in both windows, and A0$-$A4R changes sign between windows (\cref{fig:ablation}); the outcome-detail effect is large in point estimate ($+28$\,pp late) but not detectable on six tasks. The data therefore support ``history with outcome feedback beats independent attempts'' and nothing finer; because binary success is visible to every group, A0$-$A2 measures the value of the detailed feedback bundle, not of knowing whether a round succeeded.

\paragraph{Fixed and held-out layouts.} A0F has the highest late-round rate (22/36) but is scored on a seen layout: 14/16 rounds (88\%) succeed on its seen layouts against 5/16 (31\%) for A0, whereas its frozen K6 workspaces reach 27/60 (45\%) on five held-out layouts (double difference $+43.75$\,pp [$+22.5$, $+73.75$] on four tasks, with a test-channel confound; \cref{tab:app-frozen}). Fixed-layout training scores are therefore consistent with scene memorization and are not used to select a configuration. The same frozen test shows no detectable harm from reading raw prior-round records at test time: A0's K6 workspaces reach 25/60 with workspace files only and 23/60 with the raw records, $-3.3$\,pp [$-25$, $+15$] (\cref{tab:app-frozen}).
% The master doc gives the frozen contrast as "-3 pp, CI about [-17, +11]"; the repo JSON (M34) gives -3.33 [-25, +15]. Repo value used.

\paragraph{Scope.} The ablation protocol differs from the main benchmark (changing layouts, K1--K6 without a first-success stop, Astra only, six tasks): it is supporting evidence for the mechanism behind~\cref{sec:exp-curves}, not a decomposition of the main-benchmark numbers, and nothing in it transfers to the other three systems.

\subsection{Where does RSI capability come from? (outlook)}
\label{sec:exp-pca}

% The three-object explanation, the benchmark-family list, the four hypotheses and the two TODOs that
% stood here were moved to Appendix E (app:pca) via paper/integration/handoff_experiments.tex (R2 E1).
The six axes describe \emph{how} a system improves, not which abilities enable it. Following observational scaling~\cite{ruan2024observational}, we will relate the composite $\bar A$ to principal components of public benchmark scores of the same systems, keeping loadings, per-system component scores and the leave-one-out fit of $\bar A$ apart; only the fit speaks to capability sources. With four labeled systems the analysis is descriptive; the benchmark set, system set and configuration mapping are not yet frozen, so no loading is interpreted here (\cref{app:pca},~\cref{fig:pca}). Coding, spatial reasoning, logical and causal reasoning, and long-context handling are the candidate abilities, stated as hypotheses.


==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% \TODO{Conclusion to be rewritten once PCA and remaining model runs are complete}

\methodname asks a narrow question: given one zero-shot round (K0) and at most 17 self-improvement rounds (K1--K17) on 18 RoboDojo manipulation tasks, how much does a Code-as-Policy agent~\cite{liang2022codeaspolicies} improve, how fast, and at what cost. Under this protocol and limited budget, all four systems end far above their zero-shot level, and most of the gain accrues in the self-improvement rounds rather than at the switch to the workspace protocol. The systems differ less in zero-shot prior than in the speed, extent and cost of improvement; on this task set the six-axis profile and $\bar A$ place Astra above Sol and leave the Opus/Sonnet pair undecided. An Astra-only control without a workspace, on a task subset, supports reading the gains as improvement rather than resampling. These are single-chain observations of model-plus-configuration systems, not frozen capabilities: chains stop at their first success and are never re-tested, and the analysis relating $\bar A$ to public-benchmark abilities remains to be run~(\cref{app:pca}). The next steps are replicate chains, held-out re-tests of the final workspaces at benchmark scale, and further systems under matched configurations.


==> sec/6_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\paragraph{Statistical scope.} Every number rests on 18 tasks with one chain per task and system, so chain-to-chain variance for a fixed cell is unmeasured . Intervals and pairwise probabilities come from a paired task bootstrap ($B{=}5000$) and reflect task-sampling error only; no multiple-comparison correction is applied.

\paragraph{Fixed scene layout.} The main benchmark runs every round on the default layout (layout 0). The Astra ablation shows that fixed-layout training is partly scene memorization (88\% on the trained layout versus 45\% on held-out layouts), so part of the K1--K17 gain may be layout-specific; the 18-task benchmark has no held-out re-test.

\paragraph{Protocol caveats.} The K0$\to$K1 step adds a workspace and program execution before any experience exists, so it mixes tool availability with learning~(\cref{sec:exp-curves}). Independent attempts alone raise the chance of at least one success~(\cref{sec:exp-curves}); the only no-history control (A5) is Astra-only, six tasks, a different protocol; the main benchmark has no same-budget, no-memory control. Chains stop at the first native success and are never re-tested, so the curves describe observations within the budget, not a frozen capability.

\paragraph{Grader exposure.} After every round the agent receives the grader's score, success flag and failure reason and iterates on the same scene, so each chain optimizes against the grader that scores it. We did not audit chains for degenerate or grader-specific solutions.

\paragraph{Comparability across systems.} We compare ``model + configuration'' systems, not bare models: reasoning effort (high for Opus, xhigh otherwise), client (Codex CLI versus Claude Code), revision window (1800 versus 600\,s) and three task-specific hints given only to Astra differ~(\cref{app:protocol}). Truncation by the inference-time limit is uneven~(\cref{sec:exp-setup}); on the tasks untruncated for all four, Sol and Opus tie. Three Sonnet chains are unfinished, so its D2--D4 are snapshots with upper bounds.

\paragraph{Metric dependence.} D2, D3, D4 and D7 are four readings of the first-success round, so the equal-weight area counts that signal four times. We also report the cluster-downweighted area, under which the ordering is unchanged~(\cref{app:metrics}).

\paragraph{Capability-source analysis.} The pending PCA rests on public leaderboard scores of few systems at settings unlike the benchmark runs; its loadings will be descriptive and the candidate abilities remain hypotheses~(\cref{app:pca}).

\paragraph{Ablation and held-out tests.} The ablation is Astra-only, six tasks, $K\le 6$, with changing layouts and without the A4 cell, so main effects are not identifiable and the minimum detectable difference is 25--35\,pp; frozen held-out tests cover only these tasks and five layouts.

